On a notion of oplax 3-functor

We introduce a notion of normalised oplax $3$-functor suitable for the elementary homotopy theory of strict $3$-categories, following the combinatorics of orientals. We show that any such morphism induces a morphism of simplicial sets between the Street nerves and we characterise those morphisms of simplicial sets coming from normalised oplax $3$-functors. This allows us to prove that normalised oplax $3$-functors compose. Finally we construct a strictification for normalised oplax $3$-functors whose source is a $1$-category without split-monos or split-epis.

==> cellular-def_old.tex <==
    We begin this chapter by recalling the classical notion of
    \ndef{normalised oplax $2$-functor}.
    
    \begin{paragr}
     Let $A$ and $B$ be two $2$-categories.
     A \ndef{normalised oplax $2$-functor}\index{normalised oplax $2$-functor}
     $F \colon A \to B$ is given by:
     \begin{itemize}
      \item[-] a map $\Ob(A) \to \Ob(B)$ that
      to any object $x$ of $A$ associates an object
      $F(a)$ of $B$;
      \item[-] a map $\Fl_1(A) \to \Fl_1(B)$ that
      to any $1$-cell $f \colon x \to y$ of $A$ associates
      a $1$-cell $F(f) \colon F(x) \to F(y)$ of $B$;
      \item[-] a map $\Fl_2(A) \to \Fl_2(B)$ that
      to any $2$-cell $\alpha \colon f \to g$ of $A$
      associates a $2$-cell $F(\alpha) \colon F(f) \to F(g)$
      of $B$;
      \item[-] a map that to any composable $1$-cells
      $x \xrightarrow{f} y \xrightarrow{g} z$
       of $A$ associates a $2$-cell
       \[
        F(g, f) \colon F(g\comp_0 f) \to F(g) \comp_0 F(f)
       \]
       of $B$.
     \end{itemize}
     These data are subject to the following coherences:
     \begin{description}
      \item[normalisation] for any object $x$ of $A$ (resp.~any $1$-cell $f$ of $A$)
      we have $F(1_x) = 1_{F(x)}$ (resp.~$F(1_f) = 1_{F(f)}$); moreover for
      any $1$-cell $f\colon x \to y$ of $A$ we have
      \[F(1_y, f) = 1_{F(f)} = F(f, 1_x)\,;\]
      \item[cocycle] for any triple
      $x \xto{f} y \xto{g} z \xto{h} t$
      of composable $1$-cells of $A$ we have
      \[
       \bigl(F(h) \comp_0 F(g, f)\bigr) \comp_1 F(h, g\comp_0 f)
       = \bigl(F(h, g) \comp_1 F(f)\bigr) \comp_1 F(h\comp_0 g, f)\,;
      \]
      
      \item[vertical compatibility] for any pair
      \[
		 \begin{tikzcd}[column sep=4.5em]
		  a\phantom{'}
		  \ar[r, bend left=50, looseness=1.2, "f", ""{below, name=f}]
		  \ar[r, "g" description, ""{name=gu}, ""{below, name=gd}]
		  \ar[r, bend right=50, looseness=1.2, "h"', ""{name=h}]
		  \ar[Rightarrow, from=f, to=gu, "\alpha"]
		  \ar[Rightarrow, from=gd, to=h, "\beta"]&
		  a'
		 \end{tikzcd}
		\]
      of $1$-composable $2$-cells $\alpha$ and $\beta$ of $A$, we have
      $F(\beta\comp_1 \alpha) = F(\beta) \comp_1 F(\alpha)$;
      
      \item[horizontal compatibility] for any pair
      \[
      \begin{tikzcd}[column sep=4.5em]
        \bullet
        \ar[r, bend left, "f", ""{below, name=f1}]
        \ar[r, bend right, "f'"', ""{name=f2}]
        \ar[Rightarrow, from=f1, to=f2, "\alpha"]
        &
        \bullet
        \ar[r, bend left, "g", ""{below, name=g1}]
        \ar[r, bend right, "g'"', ""{name=g2}]
        \ar[Rightarrow, from=g1, to=g2, "\beta"]
        & \bullet
      \end{tikzcd}
     \]
     of $0$-composable $2$-cells $\alpha$ and $\beta$ of $A$,
     we have
     \[
      F(g', f') \comp_1 F(\beta \comp_0 \alpha) =
      \bigl( F(\beta) \comp_0 F(\alpha)\bigr) \comp_1 F(g, f)\,.
     \]
     \end{description}
    \end{paragr}
    
    \begin{paragr}
     The coherence given by the compatibility with respect to
     ``horizontal composition'' can be equivalently decomposed
     in two coherences, which correspond to the two possible
     ``whiskerings'' of a $2$-cell with a $1$-cell:
     \begin{description}
      \item[$\TreeVRight\ $] for any diagram
      \[
		 \begin{tikzcd}[column sep=4.5em]
		  a
		  \ar[r, bend left, "f", ""{below, name=f}]
		  \ar[r, bend right, "f'"', ""{name=fp}]
		  \ar[Rightarrow, from=f, to=fp, "\alpha"]
		  &
		  a' \ar[r,"g"] &
		  a''
		 \end{tikzcd}
		\]
		of $A$, we have
		\[
            F(g) \comp_0 F(\alpha) \comp_1 F(g, f)
             = 
            F(g, f') \comp_1 F(g \comp_0 \alpha)\,;
        \]
		\item[$\treeVLeft\ $] for any diagram
		\[
            \begin{tikzcd}[column sep=4.5em]
             a \ar[r, "f"] &
             a'
             \ar[r, bend left, "g", ""{below, name=g}]
		  \ar[r, bend right, "g'"', ""{name=gp}]&
		  a''
		  \ar[Rightarrow, from=g, to=gp, "\beta"]
            \end{tikzcd}
		\]
		of $A$, we have
		\[
		 F(g', f) \comp_1 F(\beta \comp_0 f)
		  =
		 F(\beta) \comp_0 F(f) \comp_1 F(g, f)\,.
		\]
     \end{description}
     These two coherences are a particular case of the horizontal coherence
     of the previous paragraph and reciprocally one checks immediately these
     two coherences joint with the vertical coherence imply the horizontal
     coherence.
     
     The advantage of this latter reformulation is that now
     the coherence datum of a normalised oplax $2$-functor
     is indexed over
     \begin{itemize}
      \item the trees of dimension $\le 2$ for the normalisation;
      \item the trees of dimension $3$ for the other coherences.
     \end{itemize}
     This will be the starting point in our generalisation towards
     a notion of normalised oplax $3$-functor.
     In order to clarify what we mean, we repropose the
     definition of normalised oplax $2$-functor
     with data and coherences indexed by trees.
    \end{paragr}
    
    \begin{paragr}
     A normalised oplax $2$-functor $F \colon A \to B$ consists
     of the following data:
     \begin{description}
		\item[$\TreeDot\:$] a map $F_{\treeDot}$ that
		to each object $a$ of $A$
		assigns an object $F_{\treeDot}(a)$ of $B$.
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
			for tree={%
				label/.option=content,
				grow'=north,
				content=,
				circle,
				fill,
				minimum size=3pt,
				inner sep=0pt,
				s sep+=15,
			}
			[[]]
			\end{forest}
		}] a map $F_{\treeLog}$ that to each $1$-cell $f \colon a \to a'$
		of $A$ assigns a $1$-cell $F_{\treeLog}(f) \colon F_{\treeDot}(a) \to F_{\treeDot}(a')$
		of $B$.
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[[][]]
			\end{forest}
		}] a map $F_{\treeV}$ that to
			to each pair of $0$\hyp{}composable $1$\hyp{}cells
			\[
			 \begin{tikzcd}
			  a \ar[r, "f"] & a' \ar[r, "g"] &  a''
			 \end{tikzcd}
			\]
			of $A$ assigns a $2$-cell $F_{\treeV}(g, f)$
			\[
			 \begin{tikzcd}[column sep=small]
				 F_{\treeDot}(a)
				 \ar[rd, "F_{\treeLog}(f)"']
				 \ar[rr, "F_{\treeLog}(g\comp_0 f)"{name=gf}] &&
				 F_{\treeDot}(a'') \\
				 & F_{\treeDot}(a') \ar[ru, "F_{\treeL}(g)"'] & 
				 \ar[Rightarrow, shorten <=1.5mm, from=gf, to=2-2]
			 \end{tikzcd}
			\]
			of $B$, that is
			\[
			 F_{\treeV}(g, f) \colon F_{\treeLog}(g \comp_0 f) \to
			 F_{\treeLog}(g) \comp_0 F_{\treeLog}(f)
			\]

			
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [ [] ] ]
			\end{forest}
		}] a map $F_{\treeLL}$
		that to each $2$-cell $\alpha \colon f \to g$ of $A$ associates
		a $2$-cell $F_{\treeLL}(\alpha) \colon F_{\treeLog}(f) \to F_{\treeLog}(g)$
		of $B$.
		\end{description}
		
		
		These data are subject to the following conditions of normalisation:
		\begin{description}
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[]
			\end{forest}
		}
		] for any object $a$ of $A$, we have
		\[
			F_{\treeLog}(1_a) = 1_{F_{\treeDot}(a)}\,;
		\]
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [] ]
			\end{forest}
		}
		] for any $1$-cell $f$ of $A$ we have
		\[
			F_{\treeLL}(1_f) = 1_{F_{\treeLog}(f)}\,;
		\]
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [] [] ]
			\end{forest}
		}
		] for any $1$\nbd-cell $f \colon a \to a'$ of $A$, we have
		\[
		 F_{\treeV}(1_{a'}, f) = F_{\treeV}(f, 1_a) = 1_{F_{\treeL}(f)}\,.
		\]
		\end{description}
		
		
		Finally, we impose the following coherences:
		\begin{description}
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[Â [] [] [] ]
			\end{forest}
		}] for any triple of $0$-composable $1$ cells
		\[
		 \begin{tikzcd}[column sep=small]
		  a \ar[r, "f"] & a' \ar[r, "g"] & a'' \ar[r, "h"] & a'''
		 \end{tikzcd}
		\]
		of $A$ we have
		\begin{center}
			\centering
			\begin{tikzpicture}[scale=2, font=\footnotesize, every label/.style={fill=white}]
			\square{%
				% Set labels.
				/square/label/.cd,
				0=$F_{\treeDot}(a)$, 1=$F_{\treeDot}(a')$, 2=$F_{\treeDot}(a'')$, 3=$F_{\treeDot}(a''')$, 
				01=${F_{\treeLog}(f)}$, 12=${F_{\treeL}(g)}$, 23=${F_{\treeL}(h)}$, 
				02=${F_{\treeL}(g\comp_0 f)}$, 03=${F_{\treeLog}(h\comp_0 g f)}$, 13=${F_{\treeL}(h g)}$,
				012=${F_{\treeV}(g, f)}$, 023={},
				123=${F_{\treeV}(h, g)}$, 013={},
				0123={$F_{\treeW}(h, g, f)$},
				/square/arrowstyle/.cd,
				0123={equal},
				/square/labelstyle/.cd,
				012={description, near start},
				123={description, near start},
				023={label={[label distance=0.15cm]-90:{\footnotesize${F_{\treeV}(h, g  f)}$}}},
				013={right, label={[label distance=0.15cm]-90:{\footnotesize${F_{\treeV}(h g, f)}$}}}
			}
			\end{tikzpicture}\ ,
		\end{center}
		that is we impose the equality
		\[
            F_{\treeLog}(h) \comp_0 F_{\treeV}(g, f) \comp_1 F_{\treeV}(h, g \comp_0 f)
		=
            F_{\treeV}(h, g) \comp_0 F_{\treeLog}(f) \comp_1 F_{\treeV}(h \comp_0 g, f)\,;
		\]
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [[][]] ]
			\end{forest}
		}] for any pair
		\[
		 \begin{tikzcd}[column sep=4.5em]
		  a\phantom{'}
		  \ar[r, bend left=50, looseness=1.2, "f", ""{below, name=f}]
		  \ar[r, "g" description, ""{name=gu}, ""{below, name=gd}]
		  \ar[r, bend right=50, looseness=1.2, "h"', ""{name=h}]
		  \ar[Rightarrow, from=f, to=gu, "\alpha"]
		  \ar[Rightarrow, from=gd, to=h, "\beta"]&
		  a'
		 \end{tikzcd}
		\]
      of $1$-composable $2$-cells $\alpha$ and $\beta$ of $A$, we impose
      \[F(\beta\comp_1 \alpha) = F(\beta) \comp_1 F(\alpha)\,;\]
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [] [[]] ]
			\end{forest}
		}] for any whiskering
		\[
		 \begin{tikzcd}[column sep=4.5em]
		  a
		  \ar[r, bend left, "f", ""{below, name=f}]
		  \ar[r, bend right, "f'"', ""{name=fp}]
		  \ar[Rightarrow, from=f, to=fp, "\alpha"]
		  &
		  a' \ar[r,"g"] &
		  a''
		 \end{tikzcd}
		\]
		of $A$ we impose
		\[
            F_{\treeLog}(g) \comp_0 F_{\treeLL}(\alpha) \comp_1 F_{\treeV}(g, f)
            =
            F_{\treeV}(g, f') \comp_1 F_{\treeLL}(g \comp_0 \alpha)\,;
        \]

		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [[]] [] ]
			\end{forest}
		}] for any whiskering
		\[
            \begin{tikzcd}[column sep=4.5em]
             a \ar[r, "f"] &
             a'
             \ar[r, bend left, "g", ""{below, name=g}]
		  \ar[r, bend right, "g'"', ""{name=gp}]&
		  a''
		  \ar[Rightarrow, from=g, to=gp, "\beta"]
            \end{tikzcd}
		\]
		of $A$ we impose
		\[
		 F_{\treeV}(g', f) \comp_1 F_{\treeLL}(\beta \comp_0 f)
		 =
		 F_{\treeLL}(\beta) \comp_0 F_{\treeLog}(f) \comp_1 F_{\treeV}(g, f)\,.
		\]
    \end{description}
    \end{paragr}
    
    \begin{paragr}
     Given two normalised oplax $2$-functors $F \colon A \to B$
     and $G \colon B \to C$, there is an obvious candidate for
     the composition $GF \colon A \to C$ and one checks that
     this is still a normalised oplax $2$-functor; furthermore,
     the identity functor on a category is clearly an identity
     element for normalised oplax $2$-functor too. Hence,
     there is a category $\widetilde{\nCat{2}}$ with small
     $2$-categories as objects and normalised oplax $2$-functors
     as morphisms.
     
     The cosimplicial object $\Delta \to \nCat{2} \to \widetilde{\nCat{2}}$
     of $\widetilde{\nCat{2}}$ induces a nerve functor
     $\widetilde{N_2} \colon \widetilde{\nCat{2}} \to \EnsSimp$.
     For any $n \ge 0$, the normalised oplax $2$-functors
     $\Deltan{n} \to A$ correspond precisely to $2$\nbd-func\-tors
     $\Onm{n}{2} \to A$
     (see, for instance, \cite[\href{https://kerodon.net/tag/00BE}{Tag 00BE}]{kerodon}).
     Hence, we get a triangle diagram of functors
     \[
     \begin{tikzcd}
      & \EnsSimp & \\
      \nCat{2} \ar[ru, "N_2"] \ar[rr, hook] &&
      \widetilde{\nCat{2}} \ar[lu, "\widetilde{N_2}"']
     \end{tikzcd}
     \]
     which is commutative (up to a canonical isomorphism). Moreover,
     it is a standard fact that the functor $\widetilde{N_2}$
     is fully faithful (see, for instance~\cite{BullejosFaroBlanco}, \cite{LackPaoli}
     or~\cite[\href{https://kerodon.net/tag/00AU}{Tag 00AU}]{kerodon}).
    \end{paragr}


\section{The cellular definition}

	Let $A$ and $B$ be two $3$-categories. We now give the
	definition of \ndef{normalised oplax $3$-functor}
	\index{normalised oplax $3$-functor}
	$F \colon A \to B$, which amounts to giving the structure
	of a family of maps indexed by the objects of $\Theta$
	of dimension at most $3$ subject to a family of relations
	indexed by the objects of $\Theta$ of dimension $4$
	as well as normalisation for identities of every dimension.
	
\begin{paragr}[Data]\label{paragr:lax_3functor_cellular_data}
    A \ndef{normalised oplax $3$-functor} $F$ from $A$ to $B$ consists
    of:
	\begin{description}
		\item[$\TreeDot\ $] a map $F_{\treeDot}$ that
		to each object $a$ of $A$
		assigns an object $F_{\treeDot}(a)$ of $B$.
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
			for tree={%
				label/.option=content,
				grow'=north,
				content=,
				circle,
				fill,
				minimum size=3pt,
				inner sep=0pt,
				s sep+=15,
			}
			[[]]
			\end{forest}
		}] a map $F_{\treeLog}$ that to each $1$-cell $f \colon a \to a'$
		of $A$ assigns a $1$-cell $F_{\treeLog}(f) \colon F_{\treeDot}(a) \to F_{\treeDot}(a')$
		of $B$;
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[[][]]
			\end{forest}
		}] a map $F_{\treeV}$ that to
			to each pair of $0$\hyp{}composable $1$\hyp{}cells
			\[
			 \begin{tikzcd}
			  a \ar[r, "f"] & a' \ar[r, "g"] &  a''
			 \end{tikzcd}
			\]
			of $A$ assigns a $2$-cell $F_{\treeV}(g, f)$
			\[
			 \begin{tikzcd}[column sep=small]
				 F_{\treeDot}(a)
				 \ar[rd, "F_{\treeLog}(f)"']
				 \ar[rr, "F_{\treeLog}(g\comp_0 f)"{name=gf}] &&
				 F_{\treeDot}(a'') \\
				 & F_{\treeDot}(a') \ar[ru, "F_{\treeL}(g)"'] & 
				 \ar[Rightarrow, shorten <=1.5mm, from=gf, to=2-2]
			 \end{tikzcd}
			\]
			of $B$, that is
			\[
			 F_{\treeV}(g, f) \colon F_{\treeLog}(g \comp_0 f) \to
			 F_{\treeLog}(g) \comp_0 F_{\treeLog}(f)\,;
			\]

			
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [ [] ] ]
			\end{forest}
		}] a map $F_{\treeLL}$
		that to each $2$-cell $\alpha \colon f \to g$ of $A$ associates
		a $2$-cell $F_{\treeLL}(\alpha) \colon F_{\treeLog}(f) \to F_{\treeLog}(g)$
		of $B$;
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[Â [] [] [] ]
			\end{forest}
		}] a map $F_{\treeW}$,
		that to each triple of $0$-composable $1$ cells
		\[
		 \begin{tikzcd}[column sep=small]
		  a \ar[r, "f"] & a' \ar[r, "g"] & a'' \ar[r, "h"] & a'''
		 \end{tikzcd}
		\]
		of $A$ associates a $3$-cell $F_{\treeW}(h, g, f)$
		\begin{center}
			\centering
			\begin{tikzpicture}[scale=1.8, font=\footnotesize, every label/.style={fill=white}]
			\square{%
				% Set labels.
				/square/label/.cd,
				0=$F_{\treeDot}(a)$, 1=$F_{\treeDot}(a')$, 2=$F_{\treeDot}(a'')$, 3=$F_{\treeDot}(a''')$, 
				01=${F_{\treeLog}(f)}$, 12=${F_{\treeL}(g)}$, 23=${F_{\treeL}(h)}$, 
				02=${F_{\treeL}(g\comp_0 f)}$, 03=${F_{\treeLog}(h\comp_0 g f)}$, 13=${F_{\treeL}(h g)}$,
				012=${F_{\treeV}(g, f)}$, 023={},
				123=${F_{\treeV}(h, g)}$, 013={},
				0123={$F_{\treeW}(h, g, f)$},
				/square/labelstyle/.cd,
				012={description, near start},
				123={description, near start},
				023={label={[label distance=0.15cm]-90:{\footnotesize${F_{\treeV}(h, g  f)}$}}},
				013={right, label={[label distance=0.15cm]-90:{\footnotesize${F_{\treeV}(h g, f)}$}}}
			}
			\end{tikzpicture}\ ,
		\end{center}
		that is the $3$-cell $F_{\treeW}(h, g, f)$ has
		\[
            F_{\treeLog}(h) \comp_0 F_{\treeV}(g, f) \comp_1 F_{\treeV}(h, g \comp_0 f)
		\]
		as source and
		\[
            F_{\treeV}(h, g) \comp_0 F_{\treeLog}(f) \comp_1 F_{\treeV}(h \comp_0 g, f)
		\]
		as target;
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [] [[]] ]
			\end{forest}
		}] a map $F_{\treeVRight}$
		that to any whiskering
		\[
		 \begin{tikzcd}[column sep=4.5em]
		  a
		  \ar[r, bend left, "f", ""{below, name=f}]
		  \ar[r, bend right, "f'"', ""{name=fp}]
		  \ar[Rightarrow, from=f, to=fp, "\alpha"]
		  &
		  a' \ar[r,"g"] &
		  a''
		 \end{tikzcd}
		\]
		of $A$ associates a $3$-cell 
		\[
            F_{\treeVRight}(g, \alpha) \colon
            F_{\treeLog}(g) \comp_0 F_{\treeLL}(\alpha) \comp_1 F_{\treeV}(g, f)
            \to
            F_{\treeV}(g, f') \comp_1 F_{\treeLL}(g \comp_0 \alpha)
        \]
        of $B$;

		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [[]] [] ]
			\end{forest}
		}] a map $F_{\treeVLeft}$,
		that to each whiskering
		\[
            \begin{tikzcd}[column sep=4.5em]
             a \ar[r, "f"] &
             a'
             \ar[r, bend left, "g", ""{below, name=g}]
		  \ar[r, bend right, "g'"', ""{name=gp}]&
		  a''
		  \ar[Rightarrow, from=g, to=gp, "\beta"]
            \end{tikzcd}
		\]
		of $A$ associates a $3$-cell
		\[
		 F_{\treeVLeft}(\beta, f) \colon
		 F_{\treeV}(g', f) \comp_1 F_{\treeLL}(\beta \comp_0 f)
		 \to
		 F_{\treeLL}(\beta) \comp_0 F_{\treeLog}(f) \comp_1 F_{\treeV}(g, f)
		\]
		of $B$;
		


		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [[[]]] ]
			\end{forest}
		}] a map $F_{\treeLLL}$,
		that to any $3$-cell $\gamma \colon \alpha \to \alpha'$ of $A$,
		\ie any tree of $A_{\treeLLL}$, associates
		a $3$-cell \[F_{\treeLLL}(\gamma) \colon F_{\treeLL}(\alpha) \to F_{\treeLL}(\alpha')\]
		of $B$.
	\end{description}
	\end{paragr}
	
	
	\begin{paragr}[Normalisation]\label{paragr:lax_3functor_cellular_norm}
		The normalisation requires the following constraints:
		\begin{description}
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[]
			\end{forest}
		}
		] for any object $a$ of $A$, we have
		\[
			F_{\treeLog}(1_a) = 1_{F_{\treeDot}(a)}\,;
		\]
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [] ]
			\end{forest}
		}
		] for any $1$-cell $f$ of $A$ we have
		\[
			F_{\treeLL}(1_f) = 1_{F_{\treeLog}(f)}\,;
		\]
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [] [] ]
			\end{forest}
		}
		] for any $1$\nbd-cell $f \colon a \to a'$ of $A$, we have
		\[
		 F_{\treeV}(1_{a'}, f) = F_{\treeV}(f, 1_a) = 1_{F_{\treeL}(f)}\,;
		\]
		
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [ []Â ] ]
			\end{forest}
		}
		] for any $2$-cell $\alpha$ of $A$ we have
		\[
		F_{\treeLLL}(1_\alpha) = 1_{F_{\treeLL}(\alpha)}\,.
		\]
		
		
		\item[%
		\scalebox{0.3}{
			\begin{forest}
				for tree={%
					label/.option=content,
					grow'=north,
					content=,
					circle,
					fill,
					minimum size=3pt,
					inner sep=0pt,
					s sep+=15,
				}
				[ [] [] [] ]
			\end{forest}
		}
		]
		for any pair $a \xto{f} a' \xto{g} a''$ of composable $1$-cell of $A$, we have
		\[
		 F_{\treeW}(g, f, 1_a) = F_{\treeW}(g, 1_{a'}, f) = F_{\treeW}(1_{a''}, g, f) = 1_{F_{\treeV}(g, f)}\,;
		\]
		
		
		
		
		\item[%
						\scalebox{0.3}{
							\begin{forest}
								for tree={%
									label/.option=content,
									grow'=north,
									content=,
									circle,
									fill,
									minimum size=3pt,
									inner sep=0pt,
									s sep+=15,
								}
								[ [] [[]] ]
							\end{forest}
						}] for any pair $a \xto{f} a' \xto{g} a''$ of composable $1$\nbd-cells
						of~$A$, we have
						\[
						F_{\treeVRight}(g, 1_f) = 1_{F_{\treeV}(g, f)}\,,
						\]
						and for any $2$-cell $\alpha \colon f \to f'$ of $A$, we have
						\[
						F_{\treeVRight}(1_{a'}, \alpha) = 1_{F_{\treeLL}(\alpha)}\,;
						\]
						
						
		\item[%
						\scalebox{0.3}{
							\begin{forest}
								for tree={%
									label/.option=content,
									grow'=north,
									content=,
									circle,
									fill,
									minimum size=3pt,
									inner sep=0pt,
									s sep+=15,
								}
								[ [[]] [] ]
							\end{forest}
						}] for any pair $a \xto{f} a' \xto{g} a''$ of composable $1$\nbd-cells
						of~$A$, we have
						\[
						F_{\treeVLeft}(1_g, f) = 1_{F_{\treeV}(g, f)}\,,
						\]
						and for any $2$-cell $\beta \colon g \to g'$ of $A$, we have
						\[
						F_{\treeVLeft}(\beta, 1_{a'}) = 1_{F_{\treeLL}(\beta)}\,;
						\]
						
		
		    
		\end{description}
		
		\end{paragr}


%
%
%
%
%
%   COHERENCES
%
%
%
%
%



	
	
	\begin{paragr}[Coherences]\label{paragr:lax_3functor_cellular_coherences}
	These maps are subject to the following relations:
	\begin{description}
	\item[%
     \scalebox{0.3}{
     	\begin{forest}
     		for tree={%
     			label/.option=content,
     			grow'=north,
     			content=,
     			circle,
     			fill,
     			minimum size=3pt,
     			inner sep=0pt,
     			s sep+=15,
     		}
     		[ [[][]] ]
     	\end{forest}
     }] for any pair of $1$-composable $2$-cells
     \[
     \begin{tikzcd}[column sep=4.5em]
     a\phantom{'}
     \ar[r, bend left=50, looseness=1.2, "f", ""{below, name=f}]
     \ar[r, "g" description, ""{name=gu}, ""{below, name=gd}]
     \ar[r, bend right=50, looseness=1.2, "h"', ""{name=h}]
     \ar[Rightarrow, from=f, to=gu, "\alpha"]
     \ar[Rightarrow, from=gd, to=h, "\beta"]&
     a'
     \end{tikzcd}
     \]
     of $A$, \ie to any tree of $A_{\treeY}$, we have an equality
     \[
     F_{\treeLL}(\beta) \comp_1 F_{\treeLL}(\alpha)
     =
     F_{\treeLL}(\beta \comp_1 \alpha)
     \]
     in $B$. We shall sometimes write $F_{\treeY}(\beta, \alpha)$
     for the identity $3$-cell of this $2$-cell above.
     
     
	 \item[%
        \scalebox{0.3}{
            \begin{forest}
                for tree={%
                    label/.option=content,
                    grow'=north,
                    content=,
                    circle,
                    fill,
                    minimum size=3pt,
                    inner sep=0pt,
                    s sep+=15,
                }
                [
                    [] [] [] []
                ]
            \end{forest}
        }
     ] For any quadruple
     \[
      \begin{tikzcd}
       \bullet \ar[r, "f"] & \bullet \ar[r, "g"] & \bullet \ar[r, "h"] & \bullet \ar[r, "i"] & \bullet
      \end{tikzcd}
     \]
     of $0$-composable $1$-cells of $A$ we impose that the $3$-cells
     \begin{gather*}
       F_{\treeV}(i, h) \comp_0 F_{\treeLog}(g) \comp_0 F_{\treeLog}(f)
       \comp_1 F_{\treeW}(ih, g, h) \\
       \comp_2\\
       F_{\treeLog}(i) \comp_0 F_{\treeLog}(h) \comp_0 F_{\treeV}(g, f)
       \comp_1 F_{\treeW}(i, h, gf)
     \end{gather*}
     and
     \begin{gather*}
       F_{\treeW}(i, h, g) \comp_0 F_{\treeLog}(f) \comp_1 F_{\treeV}(i\comp_0 h \comp_0 g, f)\\
       \comp_2\\
       F_{\treeLog}(i) \comp_0 F_{\treeV}(h, g) \comp_0 F_{\treeLog}(f) \comp_1
       F_{\treeW}(i, h \comp_0 g, f)\\
       \comp_2 \\
       F_{\treeLog}(i) \comp_0 F_{\treeW}(h, g, f) \comp_1 F_{\treeV}(i, h\comp_0 g \comp_0 f)
     \end{gather*}
     of $B$ are equal.
     
     \item[%
        \scalebox{0.3}{
            \begin{forest}
                for tree={%
                    label/.option=content,
                    grow'=north,
                    content=,
                    circle,
                    fill,
                    minimum size=3pt,
                    inner sep=0pt,
                    s sep+=15,
                }
                [
                    [ [] ] [] []
                ]
            \end{forest}
        }
     ] For any triple
     \[
      \begin{tikzcd}[column sep=4.5em]
       \bullet \ar[r, "f"] & \bullet \ar[r, "g"] &
       \bullet
       \ar[r, bend left, "h", ""{below, name=h}]
       \ar[r, bend right, "h'"', ""{name=h2}]
       \ar[Rightarrow, from=h, to=h2, "\alpha"]
       & \bullet
      \end{tikzcd}
     \]
     of $0$-composable cells $f$, $g$ and $\alpha$ of $A$
     we impose the $3$-cells
     \begin{gather*}
        F_{\treeLL}(\alpha) \comp_0 F_{\treeLog}(g) \comp_0 F_{\treeLog}(f)
        \comp_1 F_{\treeW}(h, g, f)\\
        \comp_2\\
        F_{\treeLog}(h') \comp_0 F_{\treeV}(g, f) \comp_1 F_{\treeVLeft}(\alpha, g \comp_0 f)
     \end{gather*}
     and
     \begin{gather*}
        F_{\treeVLeft}(\alpha, g) \comp_0 F_{\treeLog}(f) \comp_1 F_{\treeV}(h\comp_0 g, f)\\
        \comp_2\\
        F_{\treeV}(h', g) \comp_0 F_{\treeLog}(f) \comp_1 F_{\treeVLeft}(\alpha \comp_0 g, f)\\
        \comp_2\\
        F_{\treeW}(h', g, f) \comp_1 F_{\treeLL}(\alpha \comp_0 g \comp_0 f)
     \end{gather*}
     of $B$ to be equal.
     
     \item[%
        \scalebox{0.3}{
            \begin{forest}
                for tree={%
                    label/.option=content,
                    grow'=north,
                    content=,
                    circle,
                    fill,
                    minimum size=3pt,
                    inner sep=0pt,
                    s sep+=15,
                }
                [
                    [] [ [] ] []
                ]
            \end{forest}
        }
     ] For any triple
     \[
      \begin{tikzcd}[column sep=4.5em]
       \bullet \ar[r, "f"] &
       \bullet
       \ar[r, bend left, "g", ""{below, name=g}]
       \ar[r, bend right, "g'"', ""{name=g2}]
       \ar[Rightarrow, from=g, to=g2, "\alpha"] &
       \bullet \ar[r, "h"] & \bullet
      \end{tikzcd}
     \]
     of $0$-composable cells $f$, $\alpha$ and $h$ of $A$,
     we impose that the $3$-cells
     \begin{gather*}
        F_{\treeV}(h, g') \comp_0 F_{\treeLog}(f)
        \comp_1 F_{\treeVLeft}(h\comp_0 \alpha, f)\\
        \comp_2\\
        F_{\treeW}(h, g', f) \comp_1 F_{\treeLL}(h\comp_0 \alpha \comp_0 f)\\
        \comp_2\\
        F_{\treeLog}(h) \comp_0 F_{\treeV}(g', f) \comp_1
        F_{\treeVRight}(h, \alpha \comp_0 f)
     \end{gather*}
     and
     \begin{gather*}
        F_{\treeVRight}(h, \alpha) \comp_0 F_{\treeLog}(f)
        \comp_1 F_{\treeV}(h \comp_0 g, f)\\
        \comp_2\\
        F_{\treeLog}(h) \comp_0 F_{\treeLL}(\alpha) \comp_0 F_{\treeLog}(f)
        \comp_1 F_{\treeW}(h, g, f)\\
        \comp_2\\
        F_{\treeLog}(h) \comp_0 F_{\treeVLeft}(\alpha, f)
        \comp_1 F_{\treeV}(h, g\comp_0 f)
     \end{gather*}
     of $B$ to be equal.
     
     \item[%
        \scalebox{0.3}{
            \begin{forest}
                for tree={%
                    label/.option=content,
                    grow'=north,
                    content=,
                    circle,
                    fill,
                    minimum size=3pt,
                    inner sep=0pt,
                    s sep+=15,
                }
                [
                    [] [] [ [] ]
                ]
            \end{forest}
        }
     ] For any triple
     \[
      \begin{tikzcd}[column sep=4.5em]
       \bullet
       \ar[r, bend left, "f", ""{below, name=f}]
       \ar[r, bend right, "f'"', ""{name=f2}]
       \ar[Rightarrow, from=f, to=f2, "\alpha"] &
       \bullet \ar[r, "g"] &
       \bullet \ar[r, "h"] & \bullet
      \end{tikzcd}
     \]
     of $0$-composable cells $\alpha$, $g$ and $h$ of $A$
     we impose the $3$-cells
     \begin{gather*}
        F_{\treeV}(h, g) \comp_0 F_{\treeLog}(f')
        \comp_1 F_{\treeVRight}(h\comp_0 g, \alpha)\\
        \comp_2\\
        F_{\treeLog}(h) \comp_0 F_{\treeLog}(g) \comp_0 F_{\treeLL}(\alpha)
        \comp_1 F_{\treeW}(h, g, f)
     \end{gather*}
     and
     \begin{gather*}
        F_{\treeW}(h, g, f') \comp_1 F_{\treeLL}(h \comp_0 g \comp_0 \alpha)\\
        \comp_2\\
        F_{\treeLog}(h) \comp_0 F_{\treeV}(g, f')
        \comp_1 F_{\treeVRight}(h, g \comp_0 \alpha)\\
        \comp_2\\
        F_{\treeLog}(h) \comp_0 F_{\treeVRight}(g, \alpha)
        \comp_1 F_{\treeV}(h, g \comp_0 f)
     \end{gather*}
     of $B$ to be equal.
     
    \item[%
        \scalebox{0.3}{
            \begin{forest}
                for tree={%
                    label/.option=content,
                    grow=north,
                    content=,
                    circle,
                    fill,
                    minimum size=3pt,
                    inner sep=0pt,
                    s sep+=15,
                }
                [
                    [
                        [] []
                    ]
                    []
                ]
            \end{forest}
        }
     ] For any triple
     \[
      \begin{tikzcd}[column sep=4.5em]
       \bullet
       \ar[r, bend left=55, looseness=1.3, "f", ""{below, name=f1}]
       \ar[r, "f'"{description}, ""{name=f2u}, ""{below, name=f2d}]
       \ar[r, bend right=50, looseness=1.3, "f''"', ""{name=f3}]
       \ar[Rightarrow, from=f1, to=f2u, "\alpha"]
       \ar[Rightarrow, from=f2d, to=f3, "\beta"]
       &
       \bullet \ar[r, "g"] & \bullet
      \end{tikzcd}
     \]
     of cells $\alpha$, $\beta$ and $g$ of $A$
     we impose the equality of the $3$-cells
     \[
      F_{\treeV}(g, f'') \comp_1 F_{\treeVRight}(g, \beta \comp_1 \alpha)
     \]
     and
     \[
      F_{\treeVRight}(g, \beta) \comp_1 F_{\treeLL}(g \comp_0 \alpha)\ 
        \comp_2\ 
        F_{\treeLog}(g) \comp_0 F_{\treeLL}(\beta)
        \comp_1 F_{\treeVRight}(g, \alpha)
     \]
     of $B$.
     
     \item[%
        \scalebox{0.3}{
            \begin{forest}
                for tree={%
                    label/.option=content,
                    grow'=north,
                    content=,
                    circle,
                    fill,
                    minimum size=3pt,
                    inner sep=0pt,
                    s sep+=15,
                }
                [
                    [
                        [] []
                    ]
                    []
                ]
            \end{forest}
        }
     ] For any triple
     \[
      \begin{tikzcd}[column sep=4.5em]
        \bullet \ar[r, "f"] &
        \bullet
        \ar[r, bend left=55, looseness=1.3, "g", ""{below, name=g1}]
       \ar[r, "f'"{description}, ""{name=g2u}, ""{below, name=g2d}]
       \ar[r, bend right=50, looseness=1.3, "g''"', ""{name=g3}]
       \ar[Rightarrow, from=g1, to=g2u, "\alpha"]
       \ar[Rightarrow, from=g2d, to=g3, "\beta"]
       &
       \bullet
      \end{tikzcd}
     \]
     of cells $\alpha$, $\beta$ and $g$ of $A$ we impose
     that the $3$-cells
     \[
        F_{\treeVLeft}(\beta \comp_1 \alpha, f)
     \]
     and
     \[
        F_{\treeLL}(\beta) \comp_0 F_{\treeLog}(f)
        \comp_1 F_{\treeVLeft}(\alpha, f)\ 
        \comp_2\ 
        F_{\treeVLeft}(\beta, f) \comp_1 F_{\treeLL}(\alpha \comp_0 f)
     \]
     of $B$ to be equal.
     
     \item[%
        \scalebox{0.3}{
            \begin{forest}
                for tree={%
                    label/.option=content,
                    grow'=north,
                    content=,
                    circle,
                    fill,
                    minimum size=3pt,
                    inner sep=0pt,
                    s sep+=15,
                }
                [
                    [ [] ]
                    [ [] ]
                ]
            \end{forest}
        }
     ] Notice first that for any pair
     \[
      \begin{tikzcd}[column sep=4.5em]
        \bullet
        \ar[r, bend left, "f", ""{below, name=f1}]
        \ar[r, bend right, "f'"', ""{name=f2}]
        \ar[Rightarrow, from=f1, to=f2, "\alpha"]
        &
        \bullet
        \ar[r, bend left, "g", ""{below, name=g1}]
        \ar[r, bend right, "g'"', ""{name=g2}]
        \ar[Rightarrow, from=g1, to=g2, "\beta"]
        & \bullet
      \end{tikzcd}
     \]
     of $0$-composable $2$-cells $\alpha$ and $\beta$ of $A$,
     we have an equality of $2$-cells
     \[
      \begin{tikzcd}[column sep=-5.5em]
       \null &
       F_{\treeLL}(g' \comp_0 \alpha \comp_1  \beta \comp_0 f)
       \ar[ldd, equal, "{\treeY}"']
       = F_{\treeLL}(\beta \comp_0 f' \comp_1 g \comp_0 \alpha)
       \ar[rdd, equal, "{\treeY}"]
       & \null \\ \\
       F_{\treeLL}(g' \comp_0 \alpha) \comp_1 F_{\treeLL}(\beta \comp_0 f)
       & \null &
       F_{\treeLL}(\beta \comp_0 f') \comp_1 F_{\treeY}(g \comp_0 \alpha)
      \end{tikzcd}
     \]
     of $B$, where the equality in the higher row is just the exchange law.
     We shall denote by $F_{\text{ex}}(\beta, \alpha)$ the identity $3$-cell
     going from $F_{\treeLL}(g' \comp_0 \alpha) \comp_1 F_{\treeLL}(\beta \comp_0 f)$
     to $F_{\treeLL}(\beta \comp_0 f') \comp_1 F_{\treeY}(g \comp_0 \alpha)$.

     For any pair of $2$-cells $\alpha$ and $\beta$ of $A$
     as above, we impose the $3$-cells
     \[
        F_{\treeLL}(\beta) \comp_0 F_{\treeLog}(f')
        \comp_1 F_{\treeVRight}(g, \alpha)\ 
        \comp_2\ 
        F_{\treeLog}(g') \comp_0 F_{\treeLL}(\alpha)
        \comp_1 F_{\treeVRight}(\beta, f)
     \]
     and
     \[
        F_{\treeVLeft}(\beta, f') \comp_1 F_{\treeLL}(g\comp_0 \alpha)\ 
        \comp_2\ 
        F_{\treeV}(g', f') \comp_1 F_{\text{ex}}(\beta, \alpha)\ 
        \comp_2\ 
        F_{\treeVRight}(g', \alpha) \comp_1 F_{\treeLL}(\beta \comp_0 f)
     \]
     of $B$ to be equal. Since $F_{\text{ex}}(\beta, \alpha)$ is a trivial
     $3$-cell, this coherence is actually imposing the equality between
     the $3$-cells
     \[
      F_{\treeLL}(\beta) \comp_0 F_{\treeLog}(f')
        \comp_1 F_{\treeVRight}(g, \alpha)\ 
        \comp_2\ 
        F_{\treeLog}(g') \comp_0 F_{\treeLL}(\alpha)
        \comp_1 F_{\treeVRight}(\beta, f)
     \]
     and
     \[
        F_{\treeVLeft}(\beta, f') \comp_1 F_{\treeLL}(g\comp_0 \alpha)\ 
        \comp_2\ 
        F_{\treeVRight}(g', \alpha) \comp_1 F_{\treeLL}(\beta \comp_0 f)
     \]
     of $B$.
     
     
     
     
     
     
     
     \item[%
     \scalebox{0.3}{
     	\begin{forest}
     		for tree={%
     			label/.option=content,
     			grow'=north,
     			content=,
     			circle,
     			fill,
     			minimum size=3pt,
     			inner sep=0pt,
     			s sep+=15,
     		}
     		[
     		[
     		[] [] []
     		]
     		]
     	\end{forest}
     }
     ] For any
     triple
     \[
     \begin{tikzcd}[column sep=4.7em]
     \bullet
     \ar[r, bend left=80, looseness=1.6, ""{below, name=1}]
     \ar[r, bend left, ""{name=2u}, ""{below, name=2d}]
     \ar[r, bend right, ""{name=3u}, ""{below, name=3d}]
     \ar[r, bend right=80, looseness=1.6, ""{name=4}]
     \ar[Rightarrow, from=1, to=2u, "\alpha"]
     \ar[Rightarrow, from=2d, to=3u, "\beta"]
     \ar[Rightarrow, from=3d, to=4, "\gamma"] &
     \bullet
     \end{tikzcd}
     \]
     of $1$-composable $2$-cells $\alpha$, $\beta$ and $\gamma$
     of $A$ we have the equalities between the identity $3$-cell
     \[
     F_{\treeY}(\gamma, \beta\comp_1 \alpha) \comp_2
     F_{\treeLL}(\gamma) \comp_1 F_{\treeY}(\beta, \alpha)
     \]
     and the identity $3$-cell
     \[
     F_{\treeY}(\gamma\comp_1 \beta, \alpha) \comp_2
     F_{\treeY}(\gamma, \beta) \comp_1 F_{\treeLL}(\alpha)
     \]
     of $B$.
     
     
     \item[%
     \scalebox{0.3}{
     	\begin{forest}
     		for tree={%
     			label/.option=content,
     			grow=north,
     			content=,
     			circle,
     			fill,
     			minimum size=3pt,
     			inner sep=0pt,
     			s sep+=15,
     		}
     		[
     		[
     		[
     		[] []
     		]
     		]
     		]
     	\end{forest}
     }
     ] For any pair
     \[
     \begin{tikzcd}[column sep=7em]
     \bullet
     \ar[r, bend left=60, looseness=1.2, "\phantom{bullet}"{below, name=1}]
     \ar[r, bend right=60, looseness=1.2, "\phantom{bullet}"{name=3}]
     \ar[Rightarrow, from=1, to=3, shift right=4ex, bend right, ""{name=beta1}]
     \ar[Rightarrow, from=1, to=3, ""'{name=beta2d}, ""{name=beta2u}]
     \ar[Rightarrow, from=1, to=3, shift left=4ex, bend left, ""'{name=beta3}]
     \arrow[triple, from=beta1, to=beta2d, "\gamma"]{}
     \arrow[triple, from=beta2u, to=beta3, "\delta"]{}
     &
     \bullet
     \end{tikzcd}
     \]
     of $2$-composable $3$-cells $\gamma$ and $\delta$ of $A$ we impose
     the equality
     \[
     F_{\treeLLL}(\delta \comp_2 \gamma) = F_{\treeLLL}(\delta) \comp_2 F_{\treeLLL}(\gamma)
     \]
     between these two $3$-cells of $B$.
     
     
     \item[%
     \scalebox{0.3}{
     	\begin{forest}
     		for tree={%
     			label/.option=content,
     			grow=north,
     			content=,
     			circle,
     			fill,
     			minimum size=3pt,
     			inner sep=0pt,
     			s sep+=15,
     		}
     		[
     		[
     		[] [ []Â ]
     		]
     		]
     	\end{forest}
     }
     ] For any pair
     \[
     \begin{tikzcd}[column sep=5em]
     \bullet
     \ar[r, bend left=60, looseness=1.2, ""{below, name=1}]
     \ar[r, ""{name=2u}, ""{below, name=2d}]
     \ar[r, bend right=60, looseness=1.2, ""{name=3}]
     \ar[Rightarrow, from=1, to=2u, "\alpha"]
     \ar[Rightarrow, from=2d, to=3, shift right=2.6ex, ""{name=beta1}]
     \ar[Rightarrow, from=2d, to=3, shift left=2.6ex, ""'{name=beta2}]
     \arrow[triple, from=beta1, to=beta2, "\gamma"]{}
     &
     \bullet
     \end{tikzcd}
     \]
     of $1$-composable cells $\alpha$ and $\gamma$ of $A$, we impose that
     the $3$-cells
     \[
     F_{\treeLLL}(\gamma) \comp_1 F_{\treeLL}(\alpha)
     \]
     and
     \[
     F_{\treeLLL}(\gamma \comp_1 \alpha)
     \]
     of $B$ are equal.
     
     
     \item[%
     \scalebox{0.3}{
     	\begin{forest}
     		for tree={%
     			label/.option=content,
     			grow=north,
     			content=,
     			circle,
     			fill,
     			minimum size=3pt,
     			inner sep=0pt,
     			s sep+=15,
     		}
     		[
     		[
     		[ []Â ] []
     		]
     		]
     	\end{forest}
     }
     ] For any pair
     \[
     \begin{tikzcd}[column sep=5em]
     \bullet
     \ar[r, bend left=60, looseness=1.2, ""{below, name=1}]
     \ar[r, ""{name=2u}, ""{below, name=2d}]
     \ar[r, bend right=60, looseness=1.2, ""{name=3}]
     \ar[Rightarrow, from=2d, to=3, "\beta"]
     \ar[Rightarrow, from=1, to=2u, shift right=2.6ex, ""{name=beta1}]
     \ar[Rightarrow, from=1, to=2u, shift left=2.6ex, ""'{name=beta2}]
     \arrow[triple, from=beta1, to=beta2, "\gamma"]{}
     &
     \bullet
     \end{tikzcd}
     \]
     of $1$-composable cells $\gamma$ and $\beta$ of $A$, we impose that
     the $3$-cells
     \[
     F_{\treeLL}(\beta) \comp_1 F_{\treeLLL}(\gamma)
     \]
     and
     \[
     F_{\treeLLL}(\beta \comp_1 \gamma)
     \]
     of $B$ are equal.
     
     
    \item[%
     \scalebox{0.3}{
     	\begin{forest}
     		for tree={%
     			label/.option=content,
     			grow=north,
     			content=,
     			circle,
     			fill,
     			minimum size=3pt,
     			inner sep=0pt,
     			s sep+=15,
     		}
     		[
     		[]
     		[ [ [] ] ]
     		]
     	\end{forest}
     }
     ] For any pair
     \[
     \begin{tikzcd}[column sep=5em]
     \bullet
     \ar[r, "f"]
     &
     \bullet
     \ar[r, bend left=60, looseness=1.2, "g", "\phantom{bullet}"'{name=1}]
     \ar[r, bend right=60, looseness=1.2, "g'"', "\phantom{bullet}"{name=3}]
     \ar[Rightarrow, from=1, to=3, shift right=2ex, bend right, ""{name=beta1}]
     \ar[Rightarrow, from=1, to=3, shift left=2ex, bend left, ""'{name=beta3}]
     \arrow[triple, from=beta1, to=beta3, "\Gamma"]{}
     &
     \bullet
     \end{tikzcd}
     \]
     of $0$-composable cells $f$ and $\Gamma$ of $A$, we impose the equality
     \[
     F_{\treeV}(g', f) \comp_1 F_{\treeLLL}(\Gamma \comp_0 f) = F_{\treeLLL}(\Gamma) \comp_0 F_{\treeLog}(f) \comp_1 F_{\treeV}(g, f)
     \]
     between these two $3$-cells of $B$.
     
     
     
     \item[%
     \scalebox{0.3}{
     	\begin{forest}
     		for tree={%
     			label/.option=content,
     			grow=north,
     			content=,
     			circle,
     			fill,
     			minimum size=3pt,
     			inner sep=0pt,
     			s sep+=15,
     		}
     		[
	     		[
		     		[ [] ]
	     		]
	     		[]
     		]
     	\end{forest}
     }
     ] For any pair
     \[
     \begin{tikzcd}[column sep=5em]
     \bullet
     \ar[r, bend left=60, looseness=1.2, "f", "\phantom{bullet}"'{name=1}]
     \ar[r, bend right=60, looseness=1.2, "f'"', "\phantom{bullet}"{name=3}]
     \ar[Rightarrow, from=1, to=3, shift right=2ex, bend right, ""{name=beta1}]
     \ar[Rightarrow, from=1, to=3, shift left=2ex, bend left, ""'{name=beta3}]
     \arrow[triple, from=beta1, to=beta3, "\Gamma"]{}
     &
     \bullet
     \ar[r, "g"]
     &
     \bullet
     \end{tikzcd}
     \]
     of $0$-composable cells $\Gamma$ and $g$ of $A$, we impose the equality
     \[
	     F_{\treeV}(g, f') \comp_1 F_{\treeLLL}(g \comp_0 \Gamma) = F_{\treeLog}(g) \comp_0 F_{\treeLLL}(\Gamma) \comp_1 F_{\treeV}(g, f)
     \]
     between these two $3$-cells of $B$.
     
     
	\end{description}
	
	\begin{rem}
	 Gurski defines in~\cite{GurskiCoherence} a notion of lax trimorphism
	 between tricategories, see Definition~4.11 of~\loccit; one can easily
	 adapt anddualise suitably the definition and get a notion of
	 normalised oplax trimorphism between tricategories.
	 Consider two strict $3$-categories $A$ and $B$, 
	 a normalised oplax $3$-functor $F \colon A \to B$ and
	 a normalised oplax trimorphism $G \colon A \to B$.
	 There are two main
	 differences between Gurski's notion o normalised oplax trimorphism
	 and the notion of normalised oplax $3$-functor that we presented above.
	 \begin{itemize}
	  \item The first difference concerns the tree~$\treeY$. Gurski's
	  notion requires that, for any pair $(\beta, \alpha)$ of $1$-composable
	  $2$-cells of~$A$, there is a $3$-cell of~$B$ going from
	  $G(\beta \comp_1 \alpha)$ to $G(\beta) \comp_1 G(\alpha)$
	  which is \emph{not} invertible in general. It is essential
	  in our definition of normaised oplax $3$-functor that the
	  tree~$\treeY$ appears in the coherences. This is slightly
	  unnatural even from our arboreal point of view and it may be
	  reasonable to actually impose this condition on Gurski's
	  normalised oplax trimorphisms, in light of a comparison with
	  normalised oplax $3$-functors. Gurski calls this condition
      \emph{local strictness}. Notice that it implies in particular
      that~$F$ as well as~$G$ induce strict $2$-functors on the
      hom-$2$-categories.
	  
	  \item The second difference is deeper and somehow irreconcilable.
	  For any pair $(\beta, \alpha)$ of $0$-composable $2$-cells of~$A$,
	  the normalised oplax trimorphism provides a $3$-cell
	  \[
	   G_{\treeVLR}(\beta, \alpha) \colon 
	    G(t_1(\beta), t_1(\alpha)) \comp_1 G(\beta \comp_0 \alpha) \to
	    \bigl(G(\beta) \comp_0 G(\alpha)\bigr) \comp_1 G(s_1(\beta), s_1(\alpha))\,.
	  \]
	  This is incompatible with the algebra of the orientals.
	  In fact, a normalised oplax $3$-functor has the tree~$\treeVLR$
	  as a coherence and instead the trees~$\treeVLeft$ and~$\treeVRight$
	  as part of the data. But these pieces of data are symmetric
	  (or better dual), hence they cannot fit as a particular case
	  of a single lax or oplax datum for~$\treeVLR$.
	 \end{itemize}

	\end{rem}

	
	
	\begin{exem}\label{exem:sup}
		Let $C$ be a $3$-category. We now define a normalised oplax $3$-functor
		$\sup \colon i_{\cDelta}(N_{3}(C)) \to C$ (cf.~paragraph~\ref{paragr:slice_functor}).
		\begin{description}
			\item[$\TreeDot\ \ $] The map $\sup_{\treeDot}$ is defined by mapping
			an object $(a, x)$, where $x \colon \On{m} \to C$, to $x(\atom{m})$.
			
			\item[$\TreeLog\ \ \:$] The map $\sup_{\treeLog}$ assigns to any
			morphism $f \colon (a, x) \to (b, y)$
			of $i_{\cDelta}(N_{3}(C))$, where $x \colon \On{m} \to C$ and
			$y \colon \On{n} \to C$, the $1$-cell $x'(\atom{f(m), n})$ of $C$.
			
			\item[$\TreeV\ $] The map $\sup_{\treeV}$ assigns to any
			pair of composable morphisms
			\[
			\begin{tikzcd}
			(a, x) \ar[r, "f"] & (b, y) \ar[r, "g"] &  (c, z)
			\end{tikzcd}
			\]
			of $i_{\cDelta}(N_{3}(C))$,
			with $x \colon \On{m} \to C$, $y \colon \On{n} \to C$ and $z \colon \On{p} \to C$,
			the $2$-cell $\sup_{\treeV}(g, f)$ of $C$ given by
			\[
			z\bigl(\atom{gf(m), g(n), p}\bigr)
			\]
			
			\item[$\TreeW\ $] The map $\sup_{\treeW}$,
			assigns to any triple of composable morphisms
			\[
			\begin{tikzcd}[column sep=small]
			(a,x) \ar[r, "f"] & (b, y) \ar[r, "g"] & (c, z) \ar[r, "h"] & (d, t)
			\end{tikzcd}
			\]
			of $i_{\cDelta}(N_{3}(C))$,
			with $x \colon \On{m} \to C$, $y \colon \On{n} \to C$, $z \colon \On{p} \to C$ and
			$t \colon \On{q} \to C$,
			the $3$-cell $\sup_{\treeW}(h, g, f)$ of $C$
			given by
			\[
			t\bigl(\atom{hgf(m), hg(n), h(p), q}\bigr)
			\]
		\end{description}
		
		Notice that by definition we have that $1_{\sup_{\treeDot}(a, x)}$
		is precisely $\sup_{\treeL}(1_{(a, x)})$ and that
		the other conditions of normalisation are equally trivial by definition.
		We now check the
		coherence for the tree $\treeVV$.
		
		Consider four composable morphisms of~$i_{\cDelta}(N_{3}(C))$
		\[
		\begin{tikzcd}[column sep=small]
		(a, x) \ar[r, "f"] &
		(b, y) \ar[r, "g"] &
		(c, z) \ar[r, "h"] &
		(d, t) \ar[r, "i"] &
		(e, w)
		\end{tikzcd}\ ,
		\]
		with $x \colon \On{m} \to C$, $y \colon \On{n} \to C$, $z \colon \On{p} \to C$,
		$t \colon \On{q} \to C$ and $w \colon \On{r} \to C$.
		We have to show that the $3$-cells
		\begin{gather*}
		\textstyle
		\sup_{\treeW}(i, h, g) \comp_0 \sup_{\treeLog}(f) \comp_1\sup_{\treeV}(i\comp_0 h \comp_0 g, f)\\
		\comp_2\\
		\textstyle
		\sup_{\treeLog}(i) \comp_0 \sup_{\treeV}(h, g) \comp_0 \sup_{\treeLog}(f) \comp_1
		\sup_{\treeW}(i, h \comp_0 g, f)\\
		\comp_2 \\
		\textstyle
		\sup_{\treeLog}(i) \comp_0 \sup_{\treeW}(h, g, f) \comp_1 \sup_{\treeV}(i, h\comp_0 g \comp_0 f)
		\end{gather*}
		and
		\begin{gather*}
		\textstyle
		\sup_{\treeV}(i, h) \comp_0 \sup_{\treeLog}(g) \comp_0 \sup_{\treeLog}(f)
		\comp_1 \sup_{\treeW}(ih, g, f) \\
		\comp_2\\
		\textstyle
		\sup_{\treeLog}(i) \comp_0 \sup_{\treeLog}(h) \comp_0 \sup_{\treeV}(g, f)
		\comp_1 \sup_{\treeW}(i, h, gf)\,.
		\end{gather*}
		But these two $3$-cells are precisely the target and the source of
		the main $4$-cell of $\On{4}$ via the \oo-functor $\On{4} \xto{\phi} \On{r} \xto{w} C$,
		where
		\[
		\phi = \On{\{ihgf(m), ihg(n), ih(p), i(q), r\}}\,.
		\]
	\end{exem}
\end{paragr}


==> pent.tex <==
\makeatletter

% Setup keys for pentagon macro.
% Used to specify:
% - Labels for arrows.
% - Styles for labels and arrows.

\def\labelstylecode#1{%
  \pgfkeys@split@path%
  \edef\label@key{/pentagon/label/\pgfkeyscurrentname}%
  \edef\style@key{\pgfkeyscurrentkey/.@val}%
  \def\temp@a{#1}%
  \def\temp@b{\pgfkeysnovalue}%
  \ifx\temp@a\temp@b
    \pgfkeysgetvalue{\label@key}\temp@a
    \ifx\temp@a\temp@b\else
      \pgfkeysalso{commutative diagrams/.cd, \style@key}%
    \fi
  \else
    \pgfkeys{\style@key/.code = \pgfkeysalso{#1}}%
  \fi}
\def\arrowstylecode#1{%
  \edef\style@key{\pgfkeyscurrentkey/.@val}%
  \def\temp@a{#1}%
  \def\temp@b{\pgfkeysnovalue}%
  \ifx\temp@a\temp@b
    \pgfkeysalso{commutative diagrams/.cd, \style@key}%
  \else
    \pgfkeys{\style@key/.code = \pgfkeysalso{#1}}%
  \fi}

% Don't change these defaults here. These can be changed locally in the
% key-value list provided in a call to the pentagon of pentagons macro.

\pgfkeys{
  /pentagon/label/.cd,
  0/.initial = {$\bullet$}, 1/.initial = {$\bullet$}, 2/.initial = {$\bullet$},
  3/.initial = {$\bullet$}, 4/.initial = {$\bullet$},
  01/.initial, 12/.initial, 23/.initial, 34/.initial, 04/.initial,
  02/.initial, 03/.initial, 13/.initial, 14/.initial, 24/.initial,
  012/.initial, 013/.initial, 014/.initial, 023/.initial, 024/.initial,
  034/.initial, 123/.initial, 124/.initial, 134/.initial, 234/.initial,
  0123/.initial, 0124/.initial, 0134/.initial, 0234/.initial, 1234/.initial,
  01234/.initial,
  /pentagon/labelstyle/.cd,
  01/.@val/.initial, 12/.@val/.initial, 23/.@val/.initial, 34/.@val/.initial,
  04/.@val/.initial=\pgfkeysalso{swap},
  02/.@val/.initial=\pgfkeysalso{description},
  03/.@val/.initial=\pgfkeysalso{description},
  13/.@val/.initial=\pgfkeysalso{description},
  14/.@val/.initial=\pgfkeysalso{description},
  24/.@val/.initial=\pgfkeysalso{description},
  012/.@val/.initial=\pgfkeysalso{swap, above},
  013/.@val/.initial=\pgfkeysalso{below = 1pt},
  014/.@val/.initial=\pgfkeysalso{below},
  023/.@val/.initial=\pgfkeysalso{swap, above = 1pt},
  024/.@val/.initial=\pgfkeysalso{below left = -1pt and -1pt},
  034/.@val/.initial=\pgfkeysalso{swap, right},
  123/.@val/.initial=\pgfkeysalso{below left = -1pt and -1pt},
  124/.@val/.initial=\pgfkeysalso{swap, right},
  134/.@val/.initial=\pgfkeysalso{left},
  234/.@val/.initial=\pgfkeysalso{swap, below right = -1pt and -1pt},
  0123/.@val/.initial,
  0124/.@val/.initial=\pgfkeysalso{swap},
  0134/.@val/.initial,
  0234/.@val/.initial=\pgfkeysalso{swap},
  1234/.@val/.initial,
  01234/.@val/.initial,
  01/.code=\labelstylecode{#1}, 02/.code=\labelstylecode{#1},
  03/.code=\labelstylecode{#1}, 04/.code=\labelstylecode{#1},
  12/.code=\labelstylecode{#1}, 13/.code=\labelstylecode{#1},
  14/.code=\labelstylecode{#1}, 23/.code=\labelstylecode{#1},
  24/.code=\labelstylecode{#1}, 34/.code=\labelstylecode{#1},
  012/.code=\labelstylecode{#1}, 013/.code=\labelstylecode{#1},
  014/.code=\labelstylecode{#1}, 023/.code=\labelstylecode{#1},
  024/.code=\labelstylecode{#1}, 034/.code=\labelstylecode{#1},
  123/.code=\labelstylecode{#1}, 124/.code=\labelstylecode{#1},
  134/.code=\labelstylecode{#1}, 234/.code=\labelstylecode{#1},
  0123/.code=\labelstylecode{#1}, 0124/.code=\labelstylecode{#1},
  0134/.code=\labelstylecode{#1}, 0234/.code=\labelstylecode{#1},
  1234/.code=\labelstylecode{#1}, 01234/.code=\labelstylecode{#1},
  /pentagon/arrowstyle/.cd,
  01/.@val/.initial, 12/.@val/.initial, 23/.@val/.initial, 34/.@val/.initial,
  04/.@val/.initial, 02/.@val/.initial, 03/.@val/.initial, 13/.@val/.initial,
  14/.@val/.initial, 24/.@val/.initial,
  012/.@val/.initial=\pgfkeysalso{Rightarrow},
  013/.@val/.initial=\pgfkeysalso{Rightarrow},
  014/.@val/.initial=\pgfkeysalso{Rightarrow},
  023/.@val/.initial=\pgfkeysalso{Rightarrow},
  024/.@val/.initial=\pgfkeysalso{Rightarrow},
  034/.@val/.initial=\pgfkeysalso{Rightarrow},
  123/.@val/.initial=\pgfkeysalso{Rightarrow},
  124/.@val/.initial=\pgfkeysalso{Rightarrow},
  134/.@val/.initial=\pgfkeysalso{Rightarrow},
  234/.@val/.initial=\pgfkeysalso{Rightarrow},
  0123/.@val/.initial=\pgfkeysalso{triple},
  0124/.@val/.initial=\pgfkeysalso{triple},
  0134/.@val/.initial=\pgfkeysalso{triple},
  0234/.@val/.initial=\pgfkeysalso{triple},
  1234/.@val/.initial=\pgfkeysalso{triple},
  01234/.@val/.initial=\pgfkeysalso{quadruple},
  01/.code=\arrowstylecode{#1}, 02/.code=\arrowstylecode{#1},
  03/.code=\arrowstylecode{#1}, 04/.code=\arrowstylecode{#1},
  12/.code=\arrowstylecode{#1}, 13/.code=\arrowstylecode{#1},
  14/.code=\arrowstylecode{#1}, 23/.code=\arrowstylecode{#1},
  24/.code=\arrowstylecode{#1}, 34/.code=\arrowstylecode{#1},
  012/.code=\arrowstylecode{#1}, 013/.code=\arrowstylecode{#1},
  014/.code=\arrowstylecode{#1}, 023/.code=\arrowstylecode{#1},
  024/.code=\arrowstylecode{#1}, 034/.code=\arrowstylecode{#1},
  123/.code=\arrowstylecode{#1}, 124/.code=\arrowstylecode{#1},
  134/.code=\arrowstylecode{#1}, 234/.code=\arrowstylecode{#1},
  0123/.code=\arrowstylecode{#1}, 0124/.code=\arrowstylecode{#1},
  0134/.code=\arrowstylecode{#1}, 0234/.code=\arrowstylecode{#1},
  1234/.code=\arrowstylecode{#1}, 01234/.code=\arrowstylecode{#1}
}

% Macros to draw 2-cells.

\def\pent@abc{%
  \draw [/pentagon/arrowstyle/012] (198:0.45) --
  node [/pentagon/labelstyle/012] {
    \pgfkeysvalueof{/pentagon/label/012}} (198:0.8);
}
\def\pent@bcd{%
  \draw [/pentagon/arrowstyle/123] (126:0.45) --
  node [/pentagon/labelstyle/123] {
    \pgfkeysvalueof{/pentagon/label/123}} (126:0.8);
}
\def\pent@cde{%
  \draw [/pentagon/arrowstyle/234] (54:0.45) --
  node [/pentagon/labelstyle/234] {
    \pgfkeysvalueof{/pentagon/label/234}} (54:0.8);
}
\def\pent@ade{%
  \draw [/pentagon/arrowstyle/034] (-40:0.6) --
  node [/pentagon/labelstyle/034] {
    \pgfkeysvalueof{/pentagon/label/034}} (-5:0.5);
}
\def\pent@abe{%014
  \draw [/pentagon/arrowstyle/014] (-70:0.55) --
  node [/pentagon/labelstyle/014] {
    \pgfkeysvalueof{/pentagon/label/014}} (-110:0.55);
}
\def\pent@acd{%
  \draw [/pentagon/arrowstyle/023] (55:0.3) --
  node [/pentagon/labelstyle/023] {
    \pgfkeysvalueof{/pentagon/label/023}} (125:0.3);
}
\def\pent@bde{%
  \draw [/pentagon/arrowstyle/134] (-5:0.4) --
  node [/pentagon/labelstyle/134] {
    \pgfkeysvalueof{/pentagon/label/134}} (35:0.5);
}
\def\pent@ace{%
  \draw [/pentagon/arrowstyle/024] (-45:0.45) --
  node [/pentagon/labelstyle/024] {
    \pgfkeysvalueof{/pentagon/label/024}} (-45:0.1);
}
\def\pent@abd{%
  \draw [/pentagon/arrowstyle/013] (-90:0.22) --
  node [/pentagon/labelstyle/013] {
    \pgfkeysvalueof{/pentagon/label/013}} (-150:0.46);
}
\def\pent@bce{%
  \draw [/pentagon/arrowstyle/124] (188:0.4) --
  node [/pentagon/labelstyle/124] {
    \pgfkeysvalueof{/pentagon/label/124}} (150:0.55);
}

% Macro to draw a single pentagonal node.

\def\pent@#1#2{
  \begin{scope}[shift=#2, commutative diagrams/every diagram]

    \foreach \i in {0,1,2,3,4} {
      \tikzmath{\a = 270 - (72 * \i);}
      \node (n{#1}\i) at (\a:1) {
        \pgfkeysvalueof{/pentagon/label/\i}};
    }
    
    \node (p#1) at (0,0) [circle, inner sep = 0pt,
    fit = (n{#1}0.center)(n{#1}1.center)(n{#1}2.center)
          (n{#1}3.center)(n{#1}4.center)] {};

    \begin{scope}[commutative diagrams/.cd, every arrow, every label]
      \ifcase #1
      \def\list{0/1, 1/2, 2/3, 3/4, 0/4, 0/2, 0/3}\or
      \def\list{0/1, 1/2, 2/3, 3/4, 0/4, 1/3, 1/4}\or
      \def\list{0/1, 1/2, 2/3, 3/4, 0/4, 0/2, 2/4}\or
      \def\list{0/1, 1/2, 2/3, 3/4, 0/4, 0/3, 1/3}\or
      \def\list{0/1, 1/2, 2/3, 3/4, 0/4, 1/4, 2/4}\else
      \def\list{}\fi
      
      \foreach \s / \e in \list {
        \draw [/pentagon/arrowstyle/\s\e] (n{#1}\s) --
          node [/pentagon/labelstyle/\s\e] {
          \pgfkeysvalueof{/pentagon/label/\s\e}} (n{#1}\e);
      }
      
      \ifcase #1
      \pent@abc\pent@acd\pent@ade\or
      \pent@bcd\pent@bde\pent@abe\or
      \pent@cde\pent@ace\pent@abc\or
      \pent@ade\pent@abd\pent@bcd\or
      \pent@abe\pent@bce\pent@cde
      \else\fi

    \end{scope}
  \end{scope}
}

% The pentagon of pentagons macro itself.
%
% This is the only user callable macro provided here.
%
% Takes a single parameter consisting of a list of key value pairs. These are
% processed using the keys mechanism (pgfkeys) built into TikZ, so they follow
% a familiar format.
%
% /pentagon/label/XXX = ....      Set code to typeset label of arrow XXX
% /pentagon/arrowstyle/XXX = ...  Set TikZ format for typesetting of arrow XXX.
%                                 Overrides default.
% /pentagon/labelstyle/XXX = ...  Set TikZ format for typesetting of label on
%                                 arrow XXX. Overrides default.
%
% Here XXX denotes a sequence of integers identifying a generating cell by
% listing the numbers of the vertices (in order) of the corresponding face of
% the 4-simplex.
%
% You may use the path setting mechanism of pgfkeys to avoid too much path noise
% in a key value list. For example:
%
%   \pentagon{/pentagon/label/.cd,
%     0=$0$, 1=$1$, 2=$2$, 3=$3$, 4=$4$,
%     01=$a$, 12=$b$, 23=$c$, 34=$d$, 04=$e$,
%     02=$f$, 03=$g$, 13=$h$, 14=$k$, 24=$l$,
%     012=$\alpha$, 034=$\beta$, 023=$\gamma$, 123=$\delta$, 134=$\epsilon$,
%     014=$\zeta$, 024=$\eta$, 234=$\theta$, 013=$\iota$, 124=$\kappa$,
%     0123=$\Theta$, 0124=$\Phi$, 0134=$\Psi$, 0234=$\Lambda$, 1234=$\Pi$,
%     01234=$\mathcal{F}$}
%

\def\pentagon#1{
  \pgfkeys{#1}
  \pent@{2}{(270:3)}\pent@{0}{(198:3)}\pent@{3}{(126:3)}
  \pent@{1}{(54:3)}\pent@{4}{(342:3)}

  \begin{scope}[commutative diagrams/.cd, every arrow, every label]
    \draw [/pentagon/arrowstyle/0123] (p0) --
    node [/pentagon/labelstyle/0123] {
      \pgfkeysvalueof{/pentagon/label/0123}} (p3);

    \draw [/pentagon/arrowstyle/0134] (p3) --
    node [/pentagon/labelstyle/0134] {
      \pgfkeysvalueof{/pentagon/label/0134}} (p1);

    \draw [/pentagon/arrowstyle/1234] (p1) --
    node [/pentagon/labelstyle/1234] {
      \pgfkeysvalueof{/pentagon/label/1234}} (p4);

    \draw [/pentagon/arrowstyle/0234] (p0) --
    node [/pentagon/labelstyle/0234] {
      \pgfkeysvalueof{/pentagon/label/0234}} (p2);

    \draw [/pentagon/arrowstyle/0124] (p2) --
    node [/pentagon/labelstyle/0124] {
      \pgfkeysvalueof{/pentagon/label/0124}} (p4);

    \draw [/pentagon/arrowstyle/01234] (270:0.75) --
    node [/pentagon/labelstyle/01234] {
      \pgfkeysvalueof{/pentagon/label/01234}} (90:0.75);
  \end{scope}
}

\makeatother


==> simplicial2.tex <==
\begin{thm}
 Let $F \colon A \to B$ a normalised oplax $3$-functor.
 The morphism of simplicial sets $\Nl(F) \colon \SN(A) \to \SN(B)$
 is a simplicial oplax $3$-morphism.
\end{thm}

\begin{proof}
 The theorem is a straightforward consequence
 of the normalisation axioms.
 
 Let us show condition~\ref{cond:simpl_oplax-i}.
 Consider a $2$-cell $\alpha \colon f \to g$ of $A$ and the two normalised
 oplax $3$-functors
 $L \colon \Deltan{2} \to A$
 and $R \colon \Deltan{2} \to A$
 defined by mapping
 \begin{align*}
  \atom{01} \mapsto 1_{s_0(\alpha)} = a &,& \atom{01} \mapsto g,\\
  \atom{12} \mapsto g &,& \atom{12} \mapsto 1_{t_0(\alpha)} = a',\\
  \atom{02} \mapsto f &,& \atom{02} \mapsto f,\\
  \atom{12}\comp_0 \atom{01} \mapsto g &,& \atom{12}\comp_0 \atom{01} \mapsto g,\\
  L_{\treeV}(\atom{12}, \atom{01}) = \alpha &,&
  R_{\treeV}(\atom{12}, \atom{01} = \alpha,
 \end{align*}
 respectively, that we can depict as
 \[
  \begin{tikzcd}
   \bullet  \ar[r, "g", ""'{name=g}] & \bullet \\
   \bullet \ar[u, equal] \ar[ur, "f"', ""{name=f}]
   \ar[Rightarrow, from=f, to=1-1, shorten >=1pt, "\alpha"']
  \end{tikzcd}
  \quadet
  \begin{tikzcd}
   \bullet
   \ar[r, "g", ""'{name=g}] \ar[rd, "f"', ""{name=f}] &
   \bullet \ar[d,equal] \\
   & \bullet 
   \ar[Rightarrow, from=f, to=1-2, shorten >=1pt, "\alpha"]
  \end{tikzcd}\ .
 \]
 Now, we can view $L$ and $R$ as the $3$-face and $0$-face
 respectively of the normalised oplax $3$-functor
 $T \colon \Deltan{3} \to A$ that we can represent as
 \begin{center}
  \begin{tikzpicture}
   \square{%
    /square/label/.cd,
     0=$\bullet$, 1=$\bullet$, 2=$\bullet$, 3=$\bullet$,
     12=$g$, 02=$g$, 03=$f$, 13=$g$,
     012=$\alpha$, 023=${=}$, 123=$\alpha$, 013=${=}$,
     0123=$1_{\alpha}$,
    /square/arrowstyle/.cd,
     01={equal}, 23={equal},
     023={phantom, description}, 013={phantom, description},
     /square/labelstyle/.cd,
     023={anchor=center}, 013={anchor=center}
    }
  \end{tikzpicture}
 \end{center}
The conditions of normalisations impose that the image
under $F$ of such a diagram of $A$, \ie the image of the
normalised oplax $3$-functor $FT \colon \Deltan{3} \to B$,
must be
\begin{center}
  \begin{tikzpicture}[scale=1.5]
   \square{%
    /square/label/.cd,
     0=$\bullet$, 1=$\bullet$, 2=$\bullet$, 3=$\bullet$,
     12=$F_{\treeL}(g)$, 02=$F_{\treeL}(g)$, 03=$F_{\treeL}(f)$,
     13=$F_{\treeL}(g)$,
     012=$F_{\treeLL}(\alpha)$, 023=${=}$, 123=$F_{\treeLL}(\alpha)$, 013=${=}$,
     0123=${\Gamma}$,
    /square/arrowstyle/.cd,
     01={equal}, 23={equal},
     023={phantom, description}, 013={phantom, description},
    /square/labelstyle/.cd,
    023={anchor=center}, 013={anchor=center}
    }
  \end{tikzpicture}\ ,
\end{center}
where
\[
 \Gamma = FT_{\treeW}(\atom{23}, \atom{12}, \atom{01})\,.
\]
Now, the four $3$-cells of $B$ appearing in the definition of $\Gamma$ are
\[
 F_{\treeVLeft}(\alpha, 1_a) = 1_{F_{\treeLL}(\alpha)}\,,
\]
\[
 F_{\treeW}(1_{a'}, g, 1_a) = 1_{F_{\treeL}(g)}\,,
\]
and
\[
 F_{\treeLLL}(1_\alpha) = 1_{F_{\treeLL}(\alpha)}
\]
and
\[
 F_{\treeVRight}(1_{a'}, \alpha) = 1_{F_{\treeLL}(\alpha)}
\]
which establish condition~\ref{cond:simpl_oplax-i}.

Let us show condition~\ref{cond:simpl_oplax-ii}.
Consider the normalised oplax $3$-functor $T \colon \Deltan{3} \to A$
given by
\begin{center}
 \begin{tikzpicture}[scale=1.3]
 \square{%
 	/square/label/.cd,
 	01={}, 12={$g$}, 23={$h$}, 03={$f$}, 02={$g$}, 13={$hg$},
 	012={$=$}, 023={$\alpha$}, 013={$\alpha$}, 123={$=$},
 	0123={$1_{\alpha}$},
 	/square/arrowstyle/.cd,
 	01={equal}, 012={phantom, description}, 123={phantom, description},
 	/square/labelstyle/.cd,
 	012={anchor=center}, 123={anchor=center}
 }
 \end{tikzpicture}\ .
\end{center}
The conditions of normalisations impose that the image under $F$ of $T$ is
\begin{center}
	\begin{tikzpicture}[scale=1.5]
	\square{%
		/square/label/.cd,
		01={}, 12={$F_{\treeL}(g)$}, 23={$F_{\treeL}(h)$}, 03={$F_{\treeL}(f)$},
		02={$F_{\treeL}(g)$}, 13={$F_{\treeL}(hg)$},
		012={$=$}, 023={$F(\bar\alpha)$}, 013={$F_{\treeLL}(\alpha)$}, 123={$F_{\treeV(g, f)}$},
		0123={$\Gamma$},
		/square/arrowstyle/.cd,
		01={equal}, 012={phantom, description}, 123={phantom, description},
		/square/labelstyle/.cd,
		012={anchor=center}, 123={anchor=center}
	}
	\end{tikzpicture}\,,
\end{center}
where condition~\ref{cond:simpl_oplax-ii} gives that
$F(\bar\alpha) = F_{\treeV(g, f)} \comp_1 F_{\treeLL}(\alpha)$.
Moreover, the four main $3$-cells of $\Gamma$ are by definition
\[
 F_{\treeVLeft}(1_{hg}, 1_a) = 1_{F_{\treeLL}(hg)}\,,
\]
\[
 F_{\treeW}(h, g, 1_a) = 1_{F_{\treeV}(g, f)}\,,
\]
\[
 F_{\treeLLL}(1_{\alpha}) = 1_{F_{\treeLL}(\alpha)}
\]
and
\[
 F_{\treeVRight}(h, 1_g) = 1_{F_{\treeV(g, f)}}\,.
\]
Hence the $3$-cell $\Gamma$ is trivial and the condition~\ref{cond:simpl_oplax-ii} is verified.

Let us show condition~\ref{cond:simpl_oplax-iii}.
Consider the normalised oplax $3$-functor $T \colon \Deltan{3} \to A$
given by
\begin{center}
	\begin{tikzpicture}[scale=1.3]
	\square{%
		/square/label/.cd,
		01={$h$}, 12={$i$}, 23={}, 03={$f$}, 02={$g$}, 13={$i$},
		012={$\beta$}, 023={$\alpha$}, 013={$\beta\comp_1\alpha$}, 123={$=$},
		0123={$1_{\beta \comp_1 \alpha}$},
		/square/arrowstyle/.cd,
		01={equal}, 013={phantom, description}, 123={phantom, description},
		/square/labelstyle/.cd,
		013={anchor=center}, 123={anchor=center}
	}
	\end{tikzpicture}\ .
\end{center}
The conditions of normalisations impose that the image under $F$ of $T$ is
\begin{center}
	\begin{tikzpicture}[scale=1.5]
	\square{%
		/square/label/.cd,
		01={$F_{\treeL}(h)$}, 12={$F_{\treeL}(i)$}, 23={}, 03={$F_{\treeL}(f)$},
		02={$F_{\treeL}(g)$}, 13={$F_{\treeL}(i)$},
		012={$F(\bar\beta)$}, 023={$F_{\treeLL}(\alpha)$}, 013={$\phantom{O}F(\overline\beta\comp_1\alpha)$},
		123={},
		0123={$\Gamma$},
		/square/arrowstyle/.cd,
		01={equal}, 013={phantom, description}, 123={phantom, description},
		/square/labelstyle/.cd,
		013={anchor=center}, 123={anchor=center}
	}
	\end{tikzpicture}\,,
\end{center}
where conditions~\ref{cond:simpl_oplax-ii} and \ref{cond:simpl_oplax-iii} give
\[F(\bar\alpha) = F_{\treeV(g, f)} \comp_1 F_{\treeLL}(\alpha)\]
as well as
\[
 F(\overline\beta\comp_1\alpha) = F_{\treeV(g, f)} \comp_1 F_{\treeLL}(\beta) \comp_1 F_{\treeLL}(\alpha)\,.
\]
Moreover, the four main $3$-cells of $\Gamma$ are by definition
\[
F_{\treeVLeft}(1_{i}, h) = 1_{F_{\treeV}(i, h)}\,,
\]
\[
F_{\treeW}(1_{a''}, i, h) = 1_{F_{\treeV}(i, h)}\,,
\]
\[
F_{\treeLLL}(1_{\beta\comp_1\alpha}) = 1_{F_{\treeLL}(\beta)\comp_1 F_{\treeLL}(\alpha)}
\]
and
\[
F_{\treeVRight}(1_{a''}, \beta) = 1_{F_{\treeLL(\beta)}}\,.
\]
Hence the $3$-cell $\Gamma$ is trivial and the condition~\ref{cond:simpl_oplax-iii} is verified.
This concludes the proof of the theorem.
\end{proof}

==> square.tex <==
\makeatletter

% Setup keys for square macro.
% Used to specify:
% - Labels for arrows.
% - Styles for labels and arrows.

\def\labelstylecodes#1{%
  \pgfkeys@split@path%
  \edef\label@key{/square/label/\pgfkeyscurrentname}%
  \edef\style@key{\pgfkeyscurrentkey/.@val}%
  \def\temp@a{#1}%
  \def\temp@b{\pgfkeysnovalue}%
  \ifx\temp@a\temp@b
    \pgfkeysgetvalue{\label@key}\temp@a
    \ifx\temp@a\temp@b\else
      \pgfkeysalso{commutative diagrams/.cd, \style@key}%
    \fi
  \else
    \pgfkeys{\style@key/.code = \pgfkeysalso{#1}}%
  \fi}
\def\arrowstylecodes#1{%
  \edef\style@key{\pgfkeyscurrentkey/.@val}%
  \def\temp@a{#1}%
  \def\temp@b{\pgfkeysnovalue}%
  \ifx\temp@a\temp@b
    \pgfkeysalso{commutative diagrams/.cd, \style@key}%
  \else
    \pgfkeys{\style@key/.code = \pgfkeysalso{#1}}%
  \fi}

% Don't change these defaults here. These can be changed locally in the
% key-value list provided in a call to the morphism of squares macro.

\pgfkeys{
  /square/label/.cd,
  0/.initial = {$\bullet$}, 1/.initial = {$\bullet$}, 2/.initial = {$\bullet$},
  3/.initial = {$\bullet$},
  01/.initial, 12/.initial, 23/.initial,
  02/.initial, 03/.initial, 13/.initial,
  012/.initial, 013/.initial, 023/.initial, 123/.initial,
  0123/.initial,
  /square/labelstyle/.cd,
  01/.@val/.initial, 12/.@val/.initial, 23/.@val/.initial,
  03/.@val/.initial=\pgfkeysalso{swap},
  02/.@val/.initial=\pgfkeysalso{description},
  13/.@val/.initial=\pgfkeysalso{description},
  012/.@val/.initial=\pgfkeysalso{below left = -1pt and -1pt},
  013/.@val/.initial=\pgfkeysalso{swap, right},
  023/.@val/.initial=\pgfkeysalso{left},
  123/.@val/.initial=\pgfkeysalso{swap, below right = -1pt and -1pt},
  0123/.@val/.initial,
  01/.code=\labelstylecodes{#1}, 02/.code=\labelstylecodes{#1},
  03/.code=\labelstylecodes{#1}, 12/.code=\labelstylecodes{#1},
  13/.code=\labelstylecodes{#1}, 23/.code=\labelstylecodes{#1},
  012/.code=\labelstylecodes{#1}, 013/.code=\labelstylecodes{#1},
  023/.code=\labelstylecodes{#1}, 123/.code=\labelstylecodes{#1},
  0123/.code=\labelstylecodes{#1},
  /square/arrowstyle/.cd,
  01/.@val/.initial, 12/.@val/.initial, 23/.@val/.initial,
  02/.@val/.initial, 03/.@val/.initial, 13/.@val/.initial,
  012/.@val/.initial=\pgfkeysalso{Rightarrow},
  013/.@val/.initial=\pgfkeysalso{Rightarrow},
  023/.@val/.initial=\pgfkeysalso{Rightarrow},
  123/.@val/.initial=\pgfkeysalso{Rightarrow},
  0123/.@val/.initial=\pgfkeysalso{triple},
  01/.code=\arrowstylecodes{#1}, 02/.code=\arrowstylecodes{#1},
  03/.code=\arrowstylecodes{#1}, 12/.code=\arrowstylecodes{#1},
  13/.code=\arrowstylecodes{#1}, 23/.code=\arrowstylecodes{#1},
  012/.code=\arrowstylecodes{#1}, 013/.code=\arrowstylecodes{#1},
  023/.code=\arrowstylecodes{#1}, 123/.code=\arrowstylecodes{#1},
  0123/.code=\arrowstylecodes{#1}
}

% Macros to draw 2-cells.

\def\sq@abc{%
  \draw [/square/arrowstyle/012] (126:0.25) --
  node [/square/labelstyle/012] {
    \pgfkeysvalueof{/square/label/012}} (126:0.6);
}
\def\sq@bcd{%
  \draw [/square/arrowstyle/123] (54:0.25) --
  node [/square/labelstyle/123] {
    \pgfkeysvalueof{/square/label/123}} (54:0.6);
}
\def\sq@acd{%
  \draw [/square/arrowstyle/023] (-55:0.55) --
  node [/square/labelstyle/023] {
    \pgfkeysvalueof{/square/label/023}} (-15:0.4);
}
\def\sq@abd{%
  \draw [/square/arrowstyle/013] (235:0.55) --
  node [/square/labelstyle/013] {
    \pgfkeysvalueof{/square/label/013}} (195:0.4);
}


% Macro to draw a single square node.

\def\sq@#1#2{
  \begin{scope}[shift=#2, commutative diagrams/every diagram]

    \foreach \i in {0,1,2,3} {
      \tikzmath{\a = 225 - (90 * \i);}
      \node (n{#1}\i) at (\a:1) {
        \pgfkeysvalueof{/square/label/\i}};
    }
    
    \node (s#1) at (0,0) [circle, inner sep = 0pt,
    fit = (n{#1}0.center)(n{#1}1.center)(n{#1}2.center)
          (n{#1}3.center)] {};

    \begin{scope}[commutative diagrams/.cd, every arrow, every label]
      \ifcase #1
      \def\list{0/1, 1/2, 2/3, 0/2, 0/3}\or
      \def\list{0/1, 1/2, 2/3, 1/3, 0/3}\else
      \def\list{}\fi
      
      \foreach \s / \e in \list {
        \draw [/square/arrowstyle/\s\e] (n{#1}\s) --
          node [/square/labelstyle/\s\e] {
          \pgfkeysvalueof{/square/label/\s\e}} (n{#1}\e);
      }
      
      \ifcase #1
      \sq@abc\sq@acd\or
      \sq@abd\sq@bcd
      \else\fi

    \end{scope}
  \end{scope}
}

% The 3-simplex macro itself.
%
% This is the only user callable macro provided here.
%
% Takes a single parameter consisting of a list of key value pairs. These are
% processed using the keys mechanism (pgfkeys) built into TikZ, so they follow
% a familiar format.
%
% /square/label/XXX = ....      Set code to typeset label of arrow XXX
% /square/arrowstyle/XXX = ...  Set TikZ format for typesetting of arrow XXX.
%                                 Overrides default.
% /square/labelstyle/XXX = ...  Set TikZ format for typesetting of label on
%                                 arrow XXX. Overrides default.
%
% Here XXX denotes a sequence of integers identifying a generating cell by
% listing the numbers of the vertices (in order) of the corresponding face of
% the 4-simplex.
%
% You may use the path setting mechanism of pgfkeys to avoid too much path noise
% in a key value list. For example:
%
%   \square{/square/label/.cd,
%     0=$0$, 1=$1$, 2=$2$, 3=$3$,
%     01=$a$, 12=$b$, 23=$c$, 02=$f$, 03=$g$, 13=$h$,
%     012=$\alpha$, 023=$\beta$, 123=$\gamma$, 013=$\delta$,
%     0123=$\mathcal{F}$}
%

\def\square#1{
  \pgfkeys{#1}
  \sq@{0}{(180:1.8)}\sq@{1}{(0:1.8)}

  \begin{scope}[commutative diagrams/.cd, every arrow, every label]
    \draw [shorten >=10pt, shorten <=10pt, /square/arrowstyle/0123] (s0) --
    node [/square/labelstyle/0123] {
      \pgfkeysvalueof{/square/label/0123}} (s1);

  \end{scope}
}

\makeatother


==> square2.tex <==
\makeatletter

% Setup keys for squares macro.
% Used to specify:
% - Labels for arrows.
% - Styles for labels and arrows.

\def\labelstylecode@square#1{%
  \pgfkeys@split@path%
  \edef\label@key{/squares/label/\pgfkeyscurrentname}%
  \edef\style@key{\pgfkeyscurrentkey/.@val}%
  \def\temp@a{#1}%
  \def\temp@b{\pgfkeysnovalue}%
  \ifx\temp@a\temp@b
    \pgfkeysgetvalue{\label@key}\temp@a
    \ifx\temp@a\temp@b\else
      \pgfkeysalso{commutative diagrams/.cd, \style@key}%
    \fi
  \else
    \pgfkeys{\style@key/.code = \pgfkeysalso{#1}}%
  \fi}
\def\arrowstylecode@square#1{%
  \edef\style@key{\pgfkeyscurrentkey/.@val}%
  \def\temp@a{#1}%
  \def\temp@b{\pgfkeysnovalue}%
  \ifx\temp@a\temp@b
    \pgfkeysalso{commutative diagrams/.cd, \style@key}%
  \else
    \pgfkeys{\style@key/.code = \pgfkeysalso{#1}}%
  \fi}

% Don't change these defaults here. These can be changed locally in the
% key-value list provided in a call to the morphism of squaress macro.

\pgfkeys{
  /squares/label/.cd,
  0/.initial = {$\bullet$}, 1/.initial = {$\bullet$}, 2/.initial = {$\bullet$},
  3/.initial = {$\bullet$},
  01/.initial, 12/.initial, 23/.initial,
  02/.initial, 03/.initial, 13/.initial,
  012/.initial, 013/.initial, 023/.initial, 123/.initial,
  0123/.initial,
  /squares/labelstyle/.cd,
  01/.@val/.initial=\pgfkeysalso{swap},
  12/.@val/.initial=\pgfkeysalso{swap},
  23/.@val/.initial=\pgfkeysalso{swap},
  03/.@val/.initial,
  02/.@val/.initial=\pgfkeysalso{description},
  13/.@val/.initial=\pgfkeysalso{description},
  012/.@val/.initial=\pgfkeysalso{above left = -1pt and -1pt},
  013/.@val/.initial=\pgfkeysalso{swap, right},
  023/.@val/.initial=\pgfkeysalso{left},
  123/.@val/.initial=\pgfkeysalso{swap, above right = -1pt and -1pt},
  0123/.@val/.initial,
  01/.code=\labelstylecode@square{#1}, 02/.code=\labelstylecode@square{#1},
  03/.code=\labelstylecode@square{#1}, 12/.code=\labelstylecode@square{#1},
  13/.code=\labelstylecode@square{#1}, 23/.code=\labelstylecode@square{#1},
  012/.code=\labelstylecode@square{#1}, 013/.code=\labelstylecode@square{#1},
  023/.code=\labelstylecode@square{#1}, 123/.code=\labelstylecode@square{#1},
  0123/.code=\labelstylecode@square{#1},
  /squares/arrowstyle/.cd,
  01/.@val/.initial, 12/.@val/.initial, 23/.@val/.initial,
  02/.@val/.initial, 03/.@val/.initial, 13/.@val/.initial,
  012/.@val/.initial=\pgfkeysalso{Rightarrow},
  013/.@val/.initial=\pgfkeysalso{Rightarrow},
  023/.@val/.initial=\pgfkeysalso{Rightarrow},
  123/.@val/.initial=\pgfkeysalso{Rightarrow},
  0123/.@val/.initial=\pgfkeysalso{triple},
  01/.code=\arrowstylecode@square{#1}, 02/.code=\arrowstylecode@square{#1},
  03/.code=\arrowstylecode@square{#1}, 12/.code=\arrowstylecode@square{#1},
  13/.code=\arrowstylecode@square{#1}, 23/.code=\arrowstylecode@square{#1},
  012/.code=\arrowstylecode@square{#1}, 013/.code=\arrowstylecode@square{#1},
  023/.code=\arrowstylecode@square{#1}, 123/.code=\arrowstylecode@square{#1},
  0123/.code=\arrowstylecode@square{#1}
}

% Macros to draw 2-cells.

\def\sqs@abc{%
  \draw [/squares/arrowstyle/012] (235:0.25) --
  node [/squares/labelstyle/012] {
    \pgfkeysvalueof{/squares/label/012}} (235:0.6);
}
\def\sqs@bcd{%
  \draw [/squares/arrowstyle/123] (-54:0.25) --
  node [/squares/labelstyle/123] {
    \pgfkeysvalueof{/squares/label/123}} (-54:0.6);
}
\def\sqs@acd{%
  \draw [/squares/arrowstyle/023] (55:0.55) --
  node [/squares/labelstyle/023] {
    \pgfkeysvalueof{/squares/label/023}} (15:0.45);
}
\def\sqs@abd{%
  \draw [/squares/arrowstyle/013] (125:0.55) --
  node [/squares/labelstyle/013] {
    \pgfkeysvalueof{/squares/label/013}} (165:0.45);
}


% Macro to draw a single squares node.

\def\sqs@#1#2{
  \begin{scope}[shift=#2, commutative diagrams/every diagram]

    \foreach \i in {0,1,2,3} {
      \tikzmath{\a = 135 + (90 * \i);}
      \node (n{#1}\i) at (\a:1) {
        \pgfkeysvalueof{/squares/label/\i}};
    }

    \node (s#1) at (0,0) [circle, inner sep = 0pt,
    fit = (n{#1}0.center)(n{#1}1.center)(n{#1}2.center)
          (n{#1}3.center)] {};

    \begin{scope}[commutative diagrams/.cd, every arrow, every label]
      \ifcase #1
      \def\list{0/1, 1/2, 2/3, 0/2, 0/3}\or
      \def\list{0/1, 1/2, 2/3, 1/3, 0/3}\else
      \def\list{}\fi

      \foreach \s / \e in \list {
        \draw [/squares/arrowstyle/\s\e] (n{#1}\s) --
          node [/squares/labelstyle/\s\e] {
          \pgfkeysvalueof{/squares/label/\s\e}} (n{#1}\e);
      }

      \ifcase #1
      \sqs@abc\sqs@acd\or
      \sqs@abd\sqs@bcd
      \else\fi

    \end{scope}
  \end{scope}
}

% The 3-simplex macro itself.
%
% This is the only user callable macro provided here.
%
% Takes a single parameter consisting of a list of key value pairs. These are
% processed using the keys mechanism (pgfkeys) built into TikZ, so they follow
% a familiar format.
%
% /squares/label/XXX = ....      Set code to typeset label of arrow XXX
% /squares/arrowstyle/XXX = ...  Set TikZ format for typesetting of arrow XXX.
%                                 Overrides default.
% /squares/labelstyle/XXX = ...  Set TikZ format for typesetting of label on
%                                 arrow XXX. Overrides default.
%
% Here XXX denotes a sequence of integers identifying a generating cell by
% listing the numbers of the vertices (in order) of the corresponding face of
% the 4-simplex.
%
% You may use the path setting mechanism of pgfkeys to avoid too much path noise
% in a key value list. For example:
%
%   \squares{/squares/label/.cd,
%     0=$0$, 1=$1$, 2=$2$, 3=$3$,
%     01=$a$, 12=$b$, 23=$c$, 02=$f$, 03=$g$, 13=$h$,
%     012=$\alpha$, 023=$\beta$, 123=$\gamma$, 013=$\delta$,
%     0123=$\mathcal{F}$}
%

\def\squares#1{
  \pgfkeys{#1}
  \sqs@{0}{(180:1.8)}\sqs@{1}{(0:1.8)}

  \begin{scope}[commutative diagrams/.cd, every arrow, every label]
    \draw [shorten >=10pt, shorten <=10pt, /squares/arrowstyle/0123] (s0) --
    node [/squares/labelstyle/0123] {%
      \pgfkeysvalueof{/squares/label/0123}} (s1);

  \end{scope}
}

\makeatother
